SideSeeing: A multimodal dataset and collection of tools for sidewalk assessment

This paper introduces SideSeeing, a novel initiative that provides tools and datasets for assessing the built environment. We present a framework for street-level data acquisition, loading, and analysis. Using the framework, we collected a novel dataset that integrates synchronized video footaged captured from chest-mounted mobile devices with sensor data (accelerometer, gyroscope, magnetometer, and GPS). Each data sample represents a path traversed by a user filming sidewalks near hospitals in Brazil and the USA. The dataset encompasses three hours of content covering 12 kilometers around nine hospitals, and includes 325,000 video frames with corresponding sensor data. Additionally, we present a novel 68-element taxonomy specifically created for sidewalk scene identification. SideSeeing is a step towards a suite of tools that urban experts can use to perform in-depth sidewalk accessibility evaluations. SideSeeing data and tools are publicly available at https://sites.usp.br/sideseeing/.

==> not_related.tex <==
% This paper is unrelated to sidewalks and/or built environment
In \cite{lee2021mobilevip}, the authors developed a prototype for a mobile device designed to assist individuals with visual impairments in object detection, text reading, and facial expression recognition. The system takes input from a video camera, presents a graphical interface tailored for individuals with low vision, and delivers output through headphones. The object detector utilized is based on YOLO3 and achieves an accuracy of 96.46\% for the classes defined by the authors. Tesseract is employed for text recognition, involving a cropping operation of the region of interest in the process. A library named ``Dlib'' was used to detect faces, which are then extracted and fed into a specific network for expression recognition.

% This paper is unrelated to sidewalks and/or the built environment, but it shows an interesting point-of-view of what can be done using sensors and video combined into a single solution.
The work by \cite{adil2021motionsnap} leverages the movement sensors to automatic editing of videos.

% This paper is not about sidewalks, but is very interesting because it creates a dataset of motionless activities using IMU sensor and GPS data
\cite{pires2022dailymotionless}.

% This paper is not about sidewalks - it more user-centric
Also based on wearables, \cite{dai2023sloper4d} created a dataset obtained through LiDAR, camera and IMUs hardware. The goal was to facilitate the research of global human pose estimation with human-scene interaction in the wild.

% This paper is related to the build environment, but is not good
Other studies focus on detecting objects in a fine-grained manner, particularly within the built environment. For instance, in \cite{oyucu2022solidwastes}, the authors developed a mobile device application based on deep learning capable of detecting different ``solid wastes.'' Real-time prediction was enabled through the use of TensorFlow Lite on the mobile device. The authors obtained an accuracy of 44\%, and suggest that increasing the size of the training dataset (TACO) and reducing the number of classes may contribute to improving that number.
